Clustering Using Isoperimetric Number of Trees

In this paper we propose a graph-based data clustering algorithm which is based on exact clustering of a minimum spanning tree in terms of a minimum isoperimetry criteria. We show that our basic clustering algorithm runs in $O(n \log n)$ and with post-processing in $O(n^2)$ (worst case) time where $n$ is the size of the data set. We also show that our generalized graph model which also allows the use of potentials at vertices can be used to extract a more detailed pack of information as the {\it outlier profile} of the data set. In this direction we show that our approach can be used to define the concept of an outlier-set in a precise way and we propose approximation algorithms for finding such sets. We also provide a comparative performance analysis of our algorithm with other related ones and we show that the new clustering algorithm (without the outlier extraction procedure) behaves quite effectively even on hard benchmarks and handmade examples.

==> conclusion.tex <==
\section{Conclusion and Future Works}
we proposed an image segmentation and data clustering algorithm based  on max isoeperimetric number of weighted trees. The algorithm is efficient in running time (linear) and visual comparison of it to some other grouping algorithms shows a good performance. There is some problems which needs to be addressed here though:
\begin{itemize}
\item
What is the operational definition of outlier in clustering framework, and what is the relation of outlier in introduced framework?
\item
What is the relation of isoperimetric number of minimum spanning tree and minimum cut tree with graphs isoperimetric number? can one draw bound for graph's IPN with respect to that of these trees?
\item
Is there an efficient algorithm for graphs with low cycle space? if yes what is the relation of tree's IPN to that of graph?
\end{itemize}

==> newcommands.tex <==
\newtheorem{precor}{{\bf Corollary}}
\renewcommand{\theprecor}{{\arabic{precor}}}
\newenvironment{cor}
	{\begin{precor}
		{\hspace{-0.5 em}{\bf.\ }}}
	{\end{precor}
}
%
\newtheorem{precon}{{\bf Conjecture}}
\renewcommand{\theprecon}{{\arabic{precon}}}
\newenvironment{con}
	{\begin{precon}
		\rm{ \hspace{-0.5  em}{\bf.\ }}}
	{\end{precon}
}
%
\newtheorem{predefin}{{\bf Definition}}
\renewcommand{\thepredefin}{{\arabic{predefin}}}
\newenvironment{defin}[1]
	{\begin{predefin}
			\rm{ \hspace{-0.5  em}{\bf.\ }}{\rm #1}
			\hfill{$\spadesuit$}}
	{\end{predefin}
}
%
\newtheorem{preexm}{{\bf Example}}
\renewcommand{\thepreexm}{{\arabic{preexm}}}
\newenvironment{exm}[1]
	{\begin{preexm}
		\rm{ \hspace{-0.5  em}{\bf.\ }}{\rm #1}
		\hfill{$\clubsuit$}}
	{\end{preexm}
}
%
\newtheorem{preappl}{{\bf Application}}
\renewcommand{\thepreappl}{{\arabic{preappl}}}
\newenvironment{appl}[1]
	{\begin{preappl}
		\rm{ \hspace{-0.5  em}{\bf.\ }}{\rm #1}
		\hfill{$\blacklozenge$}}
	{\end{preappl}
}
%
\newtheorem{prelem}{{\bf Lemma}}
\renewcommand{\theprelem}{{\arabic{prelem}}}
\newenvironment{lem}
	{\begin{prelem}
		{\hspace{-0.5 em}{\bf.\ }}}
	{\end{prelem}
}
%
\newtheorem{preproof}{{\bf Proof.\ }}
\renewcommand{\thepreproof}{}
\newenvironment{proof}[1]{\begin{preproof}{\rm  #1}\hfill{$\blacksquare$}}{\end{preproof}}
%
\newtheorem{presproof}{{\bf Sketch of Proof.\ }}
\renewcommand{\thepresproof}{}
\newenvironment{sproof}[1]{\begin{presproof}{\rm  #1}\hfill{$\blacksquare$}}{\end{presproof}}
%
\newenvironment{pproof}[2]{{\bf #1.} {\rm  #2}\hfill{$\blacksquare$}}{\par}
%
\newtheorem{prethm}{{\bf Theorem}}
\renewcommand{\theprethm}{{\arabic{prethm}}}
\newenvironment{thm}{\begin{prethm}{ \hspace{-0.5  em}{\bf.\ }}}{\end{prethm}}
%
\newtheorem{prealphthm}{{\bf Theorem}}
\renewcommand{\theprealphthm}{{\Alph{prealphthm}}}
\newenvironment{alphthm}{\begin{prealphthm}\rm{ \hspace{-0.5  em}{\bf.\ }}}{\end{prealphthm}}
%
\newtheorem{preprop}{{\bf Proposition}}
\renewcommand{\thepreprop}{{\arabic{preprop}}}
\newenvironment{prop}{\begin{preprop}\rm{ \hspace{-0.5  em}{\bf.\ }}}{\end{preprop}}
%
\newenvironment{prob}[3]{\vskip 5pt
\noindent {\bf #1}\\[4pt]
\hspace*{-6pt}\begin{tabular}{p{50pt}l}
{INSTANCE:}& \parbox[t]{11.8cm}{#2}\\[7pt]
 QUERY:    & \parbox[t]{11.8cm}{#3}}
{\end{tabular}\\[5pt]}
%
\newenvironment{probc}[4]{\vskip 5pt
\noindent {\bf #1}\\[2pt]
\hspace*{-6pt}\begin{tabular}{p{58pt}l}
CONSTANTS: & \parbox[t]{11.5cm}{#2}\\[3pt]
{INSTANCE:}& \parbox[t]{11.5cm}{#3}\\
 QUERY:    & \parbox[t]{11.5cm}{#4}}{\end{tabular}\\[5pt]}
%
\def\isdef{\mbox {$\ \stackrel{\rm def}{=} \ $}}
%
\newcommand\marginlabel[1]{\mbox{}\marginpar{\raggedright\hspace{0pt}\uppercase{#1}}}
\def\thefootnote{\fnsymbol{footnote}}


\providecommand{\bysame}{\leavevmode\hbox to3em{\hrulefill}\thinspace}
\providecommand{\MR}{\relax\ifhmode\unskip\space\fi MR }

% \MRhref is called by the amsart/book/proc definition of \MR.
\providecommand{\MRhref}[2]{%
  \href{http://www.ams.org/mathscinet-getitem?mr=#1}{\MR{#2}}
}
\providecommand{\href}[2]{#2}

